GoldCoin: Grounding Large Language Models in Privacy Laws via Contextual Integrity Theory

Privacy issues arise prominently during the inappropriate transmission of information between entities. Existing research primarily studies privacy by exploring various privacy attacks, defenses, and evaluations within narrowly predefined patterns, while neglecting that privacy is not an isolated, context-free concept limited to traditionally sensitive data (e.g., social security numbers), but intertwined with intricate social contexts that complicate the identification and analysis of potential privacy violations. The advent of Large Language Models (LLMs) offers unprecedented opportunities for incorporating the nuanced scenarios outlined in privacy laws to tackle these complex privacy issues. However, the scarcity of open-source relevant case studies restricts the efficiency of LLMs in aligning with specific legal statutes. To address this challenge, we introduce a novel framework, GoldCoin, designed to efficiently ground LLMs in privacy laws for judicial assessing privacy violations. Our framework leverages the theory of contextual integrity as a bridge, creating numerous synthetic scenarios grounded in relevant privacy statutes (e.g., HIPAA), to assist LLMs in comprehending the complex contexts for identifying privacy risks in the real world. Extensive experimental results demonstrate that GoldCoin markedly enhances LLMs' capabilities in recognizing privacy risks across real court cases, surpassing the baselines on different judicial tasks.

==> tabs/evaluation_applicability.tex <==
\begin{table*}[!t]

    \renewcommand\arraystretch{1.06}
\small
    \begin{center}           
    \begin{tabular}{m{3.9cm}|m{1.0cm}<{\centering}m{1.0cm}<{\centering}|m{1.0cm}<{\centering}m{1.0cm}<{\centering}|m{1.0cm}<{\centering}m{1.0cm}<{\centering}||m{1.0cm}<{\centering}m{1.0cm}<{\centering}}
            \toprule
            \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{\textbf{MPT-7B}} &  \multicolumn{2}{c|}{\textbf{Llama2-7B}}  &\multicolumn{2}{c||}{\textbf{Mistral-7B}} & \multicolumn{2}{c}{\textbf{Llama2-13B}}  \\
            & {Acc} & {Ma-F1} & {Acc} &  {Ma-F1} & {Acc} &  {Ma-F1} & {Acc} &  {Ma-F1} \\
            \midrule
            \multicolumn{9}{l}{$\vardiamondsuit$ \emph{\textbf{Direct Prompt}}} \\
Zero-shot  &\underline{1.045}& \textbf{38.36}& 3.832& 85.11& 7.115& 95.52& 4.564& 76.03\\ 
Two-shot   & 1.047& \underline{38.41}& \underline{3.728}& \underline{84.91}& \underline{7.107}& \underline{95.40}& \underline{4.512}& \underline{75.91}\\ 
Law Recitation & \textbf{1.043} & 39.22 & \textbf{3.587} & \textbf{84.60} & \textbf{6.671} & \textbf{94.42} & \textbf{4.287} & \textbf{75.71}\\
GoldCoin & \textbf{1.043} & 39.22 & \textbf{3.587} & \textbf{84.60} & \textbf{6.671} & \textbf{94.42} & \textbf{4.287} & \textbf{75.71}\\
\midrule
            \multicolumn{9}{l}{$\vardiamondsuit$
            \emph{\textbf{\papertitle CoT}}} \\
Zero-shot  &\underline{1.045}& \textbf{38.36}& 3.832& 85.11& 7.115& 95.52& 4.564& 76.03\\ 
Two-shot   & 1.047& \underline{38.41}& \underline{3.728}& \underline{84.91}& \underline{7.107}& \underline{95.40}& \underline{4.512}& \underline{75.91}\\ 
Law Recitation & \textbf{1.043} & 39.22 & \textbf{3.587} & \textbf{84.60} & \textbf{6.671} & \textbf{94.42} & \textbf{4.287} & \textbf{75.71}\\
GoldCoin & \textbf{1.043} & 39.22 & \textbf{3.587} & \textbf{84.60} & \textbf{6.671} & \textbf{94.42} & \textbf{4.287} & \textbf{75.71}\\
            \bottomrule
    \end{tabular}
    \end{center}
    \vspace{-0.15in}
\caption{The performance of various LLMs under three settings, showing Acc and error rate across three difficulty categories and overall average. We \textbf{bold} the best results and \underline{underline} the second-best results in each setting.}
\vspace{-10pt}
    \label{tabs:applicability}
\end{table*}

==> tabs/evaluation_compliance.tex <==
\begin{table*}[!t]

    \renewcommand\arraystretch{1.06}
\small
    \begin{center}           
    \begin{tabular}{m{3.9cm}|m{1.0cm}<{\centering}m{1.0cm}<{\centering}|m{1.0cm}<{\centering}m{1.0cm}<{\centering}|m{1.0cm}<{\centering}m{1.0cm}<{\centering}||m{1.0cm}<{\centering}m{1.0cm}<{\centering}}
            \toprule
            \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{\textbf{MPT-7B}} &  \multicolumn{2}{c|}{\textbf{Llama2-7B}}  &\multicolumn{2}{c||}{\textbf{Mistral-7B}} & \multicolumn{2}{c}{\textbf{Llama2-13B}}  \\
            & {Acc} & {Ma-F1} & {Acc} &  {Ma-F1} & {Acc} &  {Ma-F1} & {Acc} &  {Ma-F1} \\
            \midrule
            \multicolumn{9}{l}{$\vardiamondsuit$ \emph{\textbf{Direct Prompt}}} \\
Zero-shot  &\underline{1.045}& \textbf{38.36}& 3.832& 85.11& 7.115& 95.52& 4.564& 76.03\\ 
Two-shot   & 1.047& \underline{38.41}& \underline{3.728}& \underline{84.91}& \underline{7.107}& \underline{95.40}& \underline{4.512}& \underline{75.91}\\ 
Law Recitation & \textbf{1.043} & 39.22 & \textbf{3.587} & \textbf{84.60} & \textbf{6.671} & \textbf{94.42} & \textbf{4.287} & \textbf{75.71}\\
GoldCoin & \textbf{1.043} & 39.22 & \textbf{3.587} & \textbf{84.60} & \textbf{6.671} & \textbf{94.42} & \textbf{4.287} & \textbf{75.71}\\
\midrule
            \multicolumn{9}{l}{$\vardiamondsuit$
            \emph{\textbf{\papertitle Instruction}}} \\
Zero-shot  &\underline{1.045}& \textbf{38.36}& 3.832& 85.11& 7.115& 95.52& 4.564& 76.03\\ 
Two-shot   & 1.047& \underline{38.41}& \underline{3.728}& \underline{84.91}& \underline{7.107}& \underline{95.40}& \underline{4.512}& \underline{75.91}\\ 
Law Recitation & \textbf{1.043} & 39.22 & \textbf{3.587} & \textbf{84.60} & \textbf{6.671} & \textbf{94.42} & \textbf{4.287} & \textbf{75.71}\\
GoldCoin & \textbf{1.043} & 39.22 & \textbf{3.587} & \textbf{84.60} & \textbf{6.671} & \textbf{94.42} & \textbf{4.287} & \textbf{75.71}\\
            \bottomrule
    \end{tabular}
    \end{center}
    \vspace{-0.15in}
\caption{The performance of various LLMs under three settings, showing Acc and error rate across three difficulty categories and overall average. We \textbf{bold} the best results and \underline{underline} the second-best results in each setting.}
\vspace{-10pt}
    \label{tabs:compliance}
\end{table*}
